Disconnection-aware Attack Detection and Isolation with Separation-based Detector Reconfiguration

This study addresses incident handling during an adverse event for dynamical networked control systems. Incident handling can be divided into five steps: detection, analysis, containment, eradication, and recovery. For networked control systems, the containment step can be conducted through physical disconnection of an attacked subsystem. In accordance with the disconnection, the equipped attack detection unit should be reconfigured to maintain its detection capability. In particular, separating the detection subunit associated with the disconnected subsystem is considered as a specific reconfiguration scheme in this study. This paper poses the problem of disconnection-aware attack detection and isolation with the separation-based detector reconfiguration. The objective is to find an attack detection unit that preserves its detection and isolation capability even under any possible disconnection and separation. The difficulty arises from network topology variation caused by disconnection that can possibly lead to stability loss of the distributed observer inside the attack detection unit. A solution is proposed based on an existing controller design technique referred to as retrofit control. Furthermore, an application to low-voltage power distribution networks with distributed generation is exhibited. Numerical examples evidence the practical use of the proposed method through a benchmark distribution network.

==> doublestroke/README <==

Doublestroke Font V1.111         27th of August, 2002
------------------------

This font is based on the Computer Modern Roman family of fonts
by D. E. Knuth. It is useful for typesetting the mathematical
symbols for the natural numbers (N), whole numbers (Z),
rational numbers (Q), real numbers (R) and complex numbers (C).


License
-------

You may use and distribute these fonts as you like.
You may modify these fonts as long as you do not
rename the files to one of those names that 
Donald E. Knuth chose for the Computer Modern fonts.
(And seriously, who would want to do that?)


How to Install
--------------

1. If a previous version of this font is installed, remove all
the files, especially the font files that were generated by
Metafont after the first installation.

2. Depending on how you obtained this package it might be
necessary to unpack/uncompress an archive. Now the files

             dsrom12.pfb  dsss10.mf   dsss8.tfm
dsdoc.pdf    dsrom12.tfm  dsss10.pfb  dstroke.map
dsdoc.tex    dsrom8.mf    dsss10.tfm  readme
dsfont.sty   dsrom8.pfb   dsss12.mf   Udsrom.fd
dsrom10.mf   dsrom8.tfm   dsss12.pfb  Udsss.fd
dsrom10.pfb  dsrom.mf     dsss12.tfm
dsrom10.tfm  dsromo.mf    dsss8.mf
dsrom12.mf   dsromu.mf    dsss8.pfb

should be present.

3. Make sure you have TeX, LaTeX (with NFSS), and Metafont
installed. Make sure that cmbase.mf is accessible by Metafont.

4. Move the files to their destination.

The files        are                     and are needed by
    *.tfm        TeX font metric files   TeX
    *.fd         font defintions         TeX
    *.sty        style files             TeX
    *.mf         Metafont sources        Metafont

The exact location where the files belong depends on your
installation. As a first approximation, install them
near other files with the same extension.

5. Verify the installation by generating the documentation.
Run `latex dsdoc' and have a look at the file dsdoc.dvi which
contains the documentation and usage samples.

6. If you want to use the PostScript fonts, you have to make
them known to dvips and/or PDFTeX. The details of
this process depend on your system installation,
typically using the mapping information from the
file dstroke.map and following further instructions
contained in the main manual.

7. After reading the examples in the file dsdoc you can
use the fonts in your own documents.



After the Installation
----------------------

Do not worry, most installations complete without any problems.
However, if the procedure described above does not work, I suggest
the following actions:
  - If LaTeX complains about a missing input file, check whether
    the files *.fd and *.sty are accessible and readable.
  - If LaTeX complains about a missing font, check the
    placement of the files *.tfm .
  - If LaTeX issues strange errors, you might have an old version
    of LaTeX or NFSS. Try using the fonts with low-level font
    commands instead of dsfont.sty and check the next item, too.
  - If LaTeX issues strange errors, the files might have been
    corrupted during transmission. Conversions of CR, LF, and
    so on might cause this problem.
  - If the previewer or the printer driver complains about missing
    fonts and does not automatically call Metafont to generate
    these font, either adapt your installation or generate
    the fonts by hand. Depending on your installation you
    must run something like
      mf '\mode=localfont; input dsrom10'
    for each of the fonts.
  - If Metafont is called and complains about missing source
    files, check whether these (*.mf) are placed correctly.
  - If Metafont is called and complains about strange paths
    or about paths that do not intersect, you are probably
    generating the font at a lower resolution than 100 dpi.
    There is little you can do except ignoring the errors or
    telling Metafont to do so. Please report such errors only
    if they occur at resolutions above 100 dpi.
  - If the previewer or the printer driver complains about missing
    characters, check whether you have deleted all files from
    previous versions of this font.
  - If the previewer or the printer driver complains about a
    checksum error, check whether you have deleted all files from
    previous versions of this font.

If that does not help and your friendly TeXnician is unavailable,
drop me a mail. I will try to help you, if time permits.

I am always glad to hear about improvements and bug reports,
general comments are appreciated, too.

Olaf Kummer

Universitaet Hamburg
Fachbereich Informatik -- Arbeitsbereich TGI
Vogt-Koelln-Strasse 30
22527 Hamburg (Germany)

mailto:kummer@informatik.uni-hamburg.de
http://www.informatik.uni-hamburg.de/TGI/mitarbeiter/wimis/kummer.html

